Natural Deduction and the Isabelle Proof Assistant

We describe our Natural Deduction Assistant (NaDeA) and the interfaces between the Isabelle proof assistant and NaDeA. In particular, we explain how NaDeA, using a generated prover that has been verified in Isabelle, provides feedback to the student, and also how NaDeA, for each formula proved by the student, provides a generated theorem that can be verified in Isabelle.

==> eptcsdata.tex <==
\providecommand{\firstpage}{140}
\providecommand{\publicationstatus}{P. Quaresma and W. Neuper (Eds.): 6th International Workshop\\ on Theorem proving components for Educational software (ThEdu'17)\\
EPTCS 267, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.267.9}{10.4204/EPTCS.267.9}}
\pdfoutput=1

